Orienting Point Clouds with Dipole Propagation

Establishing a consistent normal orientation for point clouds is a notoriously difficult problem in geometry processing, requiring attention to both local and global shape characteristics. The normal direction of a point is a function of the local surface neighborhood; yet, point clouds do not disclose the full underlying surface structure. Even assuming known geodesic proximity, calculating a consistent normal orientation requires the global context. In this work, we introduce a novel approach for establishing a globally consistent normal orientation for point clouds. Our solution separates the local and global components into two different sub-problems. In the local phase, we train a neural network to learn a coherent normal direction per patch (i.e., consistently oriented normals within a single patch). In the global phase, we propagate the orientation across all coherent patches using a dipole propagation. Our dipole propagation decides to orient each patch using the electric field defined by all previously orientated patches. This gives rise to a global propagation that is stable, as well as being robust to nearby surfaces, holes, sharp features and noise.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> figures/aliens/alien_128.tex <==
\begin{figure}[h]
    \centering
    \newcommand{\pl}{-4.0}
    \begin{overpic}[width=\columnwidth]{figures/aliens/alien_128.jpg}
    \put(15,  \pl){\textcolor{black}{König}}
    \put(45,  \pl){\textcolor{black}{PCP-Net}}
    \put(80,  \pl){\textcolor{black}{Ours}}
    \end{overpic}
    \caption{Normal orientation estimation, where errors are visualized in a heat map. The MST-based technique of~\shortcite{Knig2009ConsistentPO} fails at some point in the propagation, which results in a large region of accumulated errors.}
    \label{fig:aliens_comparison}
\end{figure}


==> scratch.tex <==
todo:
1. forward reference related work of volumetric methods
2. 





\input{figures/2D/baby_shark/baby_shark_hoppe}

\section{Method}

\subsection{Patching}
First the point cloud is scaled to a unit cube, and divided into patches corresponding to 3D cubical voxels. The width of each voxel is a hyper-parameter and we observed that $\frac{1}{25}$ works well in our experiments. After discarding empty voxel regions and merging patches smaller than $100$ points, we are left with a total of ${\sim}100$ patches. 

We filter out planar patches since they are trivial to coherently orient (\emph{e.g.,} via a point on either side of the plane). We calculate the smallest eigenvalue per-patch, where near-zero eigenvalue indicates a plane. We observed that filtering values lower than $0.00015$ resulted in desirable filtering of planar patches. After this stage, ${\sim}70$ out of ${\sim}100$ patches are classified as planar, and the remaining ${\sim}30$ patches are coherently oriented by the neural network.

\subsection{Coherent Neural Patch Orientation}
We train a network on the non-planar patches, which contain the challenging cases of cavities, non-convex, and sharp feature regions. During both training and inference, we calculate normals for each point in the patch using an off-the-shelf tool (\emph{e.g.,} PCA or Jets~\cite{cazals2005estimating}), and then orient them in the direction of their center of mass. This simple orientation approach will inevitably result in incoherent normal orientations, which the neural network learns to fix. We use a PointCNN~\cite{li2018pointcnn}-based network to predict a probability per point in the patch whether it should be flipped.


The input to the network is a patch $\mathbb{P} \in \mathbb{R}^{N\times6}$, represented as a collection of $N$ points containing the xyz positions and normal direction for each point. We place each patch in a canonical pose, by rotating each patch by its PCA eigenvector, and scale the highest eigenvalue to give $1$. The output of the network $\in \mathbb{R}^{N\times2}$ is two logits per point, which when passed to Softmax result in the $flip$ probability. The network is trained using a supervision, using the cross-entropy between the predicted probabilities and the ground-truth $flip$ labels.

\subsubsection{Ensemble Training.}
We train an ensemble of point neural networks to predict flip probabilities per point. Each neural network in the ensemble can be trained with different network hyper-parameters and on different datasets. After training is complete, we average the probabilities from the different networks to obtain the final flip probability per-point. After flipping each normal according to the network-predicted probabilities the result is a coherently oriented patch.

Learning to predict a coherent normal orientation per point requires consideration of \textit{both} nearby and far away points in the patch, which we address using an ensemble of multi-scale networks. The \emph{receptive-field} of the neural network  naturally dictates the amount of far away points. We obtain networks with a large receptive field by using an aggressive pooling strategy. Each network is composed of PointCNN convolution layers, FPS (farthest-point sampling) pooling, and feature interpolation unpooling. 
Our aggressive pooling strategy uses four FPS pooling layers, where each layer reduces the number of points by 40\%. More details about our network architecture can be found in the experimental results section.

\input{figures/patch_overview}

We generate training data using self-supervision, by generating point clouds from the patches of ${\sim}100$ different (oriented) meshes. We use several forms of data augmentation to enrich the training set. During training, we flip each normal in the patch with probability $p$, where $p \sim U(0,1)$. This introduces uncorrelated local flip error that can be induced by noisy points, for example. 
We initially orient the estimated normals in each patch to point away from a single \emph{reference} point. During inference, the reference point is the center of mass. However, in order to induce different types of training distributions, we randomly select different reference points within the bounding box containing the patch. This augmentation generates spatially correlated flip errors. For example, in a patch that contains a corner, changing the reference point to be above or inside the corner will result in two different orientations for the perpendicular planes.

The strict definition of a coherently oriented patch has two valid possibilities. However, training on the best of both options (\emph{i.e.,} min-distance) is non-smooth, and can oscillate between optima. In addition, this would enable the network to \textit{memorize} spatial layouts of point patches (completely ignoring the input normal information), and always predict in the $+z$ direction, for example. Therefore, during training, we define a \textit{correct} coherent orientation based on the direction of the \textit{majority} of the estimated point normal directions. 
Orienting point normals in the same input patch using different reference points can lead to different majority normal directions, which will result in a different ground-truth label.



























 







\subsubsection{Electric Dipole}
In electrostatics, an electric dipole arises when two charged particles with opposite charge are brought close together.
The polarization of the dipole is defined to be the unit vector from the negative charge to the positive charge multiplied by their charge magnitude. In our case, the polarization is analogous to a point together with its oriented normal.
The \textit{potential} created by such dipole is a solution to the Poisson equation, and has two important properties which are desirable for propagating normal orientation: 

\begin{enumerate}
\item decreases with distance, and
\item negative on one side of the dipole and positive on the other.
\end{enumerate}

Property (1) is important such that we have a higher chance of propagating to near by points which we can be more certain about.
Property (2) helps decide the orientation of new points from already oriented points in an iterative manner, such that we point new normals from low to high potential.


Yet, dipoles are not the only technique which provides the above properties. The reasoning for using electrical dipoles is justified by the Poisson equation. In each step of our propagation we assume the orientation of previously oriented points, and want to use them to orient new points. In other words, the oriented points are the boundary conditions, and we wish to create a smooth \textit{well-behaved} \textit{potential} to decide the orientation of new points.
The solution to such a \textit{well-behaved} functional that satisfies minimum oscillations is the Poisson equation. 

Moreover, \cite{Barill:FW:2018} recently showed that the \textit{potential} dissipated from the superposition of such dipoles is the winding number function. Indeed, for shapes with oriented normals the winding number indicates whether a point in space is inside or outside a closed surface. After dipole propagation, the final \textit{potential} converges to the winding number solution.

In addition, using this function allows for a fast computation of the potential and its gradient at each point. Both the potential and its gradient can be analytically derived at each point, without the need to voxelize the space and numerically evaluate the potential at each point. Furthermore equation~\ref{eq:superposition_equation} allow us to incrementally add the effect of new oriented points to the total potential without reevaluating it each step of the propagation. 

\subsubsection{Dipole Field and Potential}
The potential $u$ generated by a dipole measured at point $\vec{r}$ is:
\begin{equation}
    u(\vec{r})= \frac{\vec{p}\cdot \vec{r}}{4\pi \cdot \mid \vec{r} \mid^3 }
    \label{eq:dipole_potential}
\end{equation}

where $\vec{p}$ is the polarization of the dipole, in our case the normal vector of each point, and $\vec{r}$ the displacement vector to the dipole, or distance from the source point in our case.

Accordingly, the electric field is the gradient of $u$:

\begin{equation}
    \vec{E} = \vec{\nabla}u(\vec{r}) = \frac{3(\vec{p}\cdot \hat{r})\hat{r} - \vec{p}}{4\pi\cdot \mid \vec{r}\mid^3}
    \label{eq:dipole_field}
\end{equation}

Note this is actually the electric field in physics up to a sign, in real physics $\vec{E}=-1 \cdot \vec{\nabla}u(\vec{r}) $, we take $\vec{E}=\vec{\nabla}u(\vec{r})$ without the minus sign, because we care to orient points towards where the potential rises, rather than falls. 
This would be the same as saying opposite charges repel instead of attract, which is opposite from real physics, but desirable in our case. 

\subsubsection{Potential Energy}
The potential energy between a patch and the currently dissipated field from previously oriented points is:


\begin{equation}
    V_{patch} = \sum_{\vec{p_i} \in patch } \vec{p_i} \cdot \vec{E}
    \label{eq:potential_energy}
\end{equation}

To account for the certainty score the network has in any point $i$, we scale the vector $\vec{p_i}$ from Equation~\ref{eq:potential_energy} by the confidence score of the network. That way points with low fidelity have lower effect on the potential energy between the patches, such that they are most likely to be oriented towards the end and have lower effect on the overall field in general.


\subsection{Diffusion}
After the patches have been oriented by the dipole propagation, we can do an extra step to fix small coherency error that the network made.
For each patch we evaluate the field effect all other patches have on it, and flip points that don't agree with that field. This is a bit similar to erosion and dilation done for 2D images. Although we used this step in our examples it is not mandatory and doesn't have to be used for super complicated or large patches.













